Artificial Intelligence for Prosthetics - challenge solutions

In the NeurIPS 2018 Artificial Intelligence for Prosthetics challenge, participants were tasked with building a controller for a musculoskeletal model with a goal of matching a given time-varying velocity vector. Top participants were invited to describe their algorithms. In this work, we describe the challenge and present thirteen solutions that used deep reinforcement learning approaches. Many solutions use similar relaxations and heuristics, such as reward shaping, frame skipping, discretization of the action space, symmetry, and policy blending. However, each team implemented different modifications of the known algorithms by, for example, dividing the task into subtasks, learning low-level control, or by incorporating expert knowledge and using imitation learning.

==> sections2018/00_intro.tex <==
\section{Introduction}

Recent advancements in material science and device technology have increased interest in creating prosthetics for improving human movement. Designing these devices, however, is difficult as it is costly and time-consuming to iterate through many designs. This is further complicated by the large variability in response among many individuals. One key reason for this is that our understanding of the interactions between humans and prostheses is not well-understood, which limits our ability to predict how a human will adapt his or her movement. Physics-based, biomechanical simulations are well-positioned to advance this field as it allows for many experiments to be run at low cost. Recent developments in using reinforcement learning techniques to train realistic, biomechanical models will be key in increasing our understanding of the human-prosthesis interaction, which will help to accelerate development of this field.

%Human movement results from the intricate coordination of muscles, tendons, joints, and other physiological elements. While children learn to walk, run, climb, and jump in their first years of life and most of us can navigate complex environments--like a crowded street or moving subway--without considerable active attention, developing controllers that can efficiently and robustly synthesize realistic human motions in a variety of environments remains a grand challenge for biomechanists, neuroscientists, and computer scientists. Current controllers are confined to a small set of pre-specified movements or driven by torques, rather than the complex muscle actuators found in humans.

In this competition, participants were tasked with developing a controller to enable a physiologically-based human model with a prosthetic leg to move at a specified direction and speed. Participants were provided with a human musculoskeletal model and a physics-based simulation environment (OpenSim \cite{delp2007opensim,seth2018opensim}) in which they synthesized physically and physiologically accurate motion (Figure \ref{fig:running}). Entrants were scored based on how well the model moved according to the requested speed and direction of walking. We provided competitors with a parameterized training environment to help build the controllers, and competitors' scores were based on a final environment with unknown parameters.

%The benefits of the challenge range across multiple domains. 

This competition advanced and popularized an important class of reinforcement learning problems, characterized by a large set of output parameters (human muscle controls) and a comparatively small dimensionality of the input (state of a dynamic system). Our challenge attracted over 425 teams from the computer science, biomechanics, and neuroscience communities, submitting 4,575 solutions. Algorithms developed in this complex biomechanical environment generalize to other reinforcement learning settings with highly-dimensional decisions, such as robotics, multivariate decision making (corporate decisions, drug quantities), and the stock exchange.

In this introduction, we first discuss state-of-the-art research in motor control modeling and simulations as a tool for solving problems in biomechanics (Section \ref{ss:scope}). Next, we specify the details of the task and performance metrics used in the challenge (Section \ref{ss:task}). Finally, we discuss results of the challenge and provide a summary of the common strategies that teams used to be successful in the challenge (Section \ref{ss:solutions}). In the following sections, top teams describe their approaches in more detail.

%This challenge also directly benefited the biomechanics and neuroscience communities. The control models trained could be extended, for example, to a clinical setting to help predict how a patient will walk after surgery. The controllers developed may also potentially approximate human motor control and thus deepen our understanding of human movement. Reinforcement learning is also a powerful tool for identifying deficiencies and errant assumptions made when building models, thus the challenge will also improve on the current state-of-the-art for computational musculoskeletal modeling.

%The competition is designed for participants to use reinforcement learning methods to create their controllers. However, unlike in pure reinforcement learning tasks, we will allow participants to use publicly available human movement data. As the benchmark, we will use state-of-the art reinforcement learning techniques such as Proximal Policy Optimization (PPO) and Deep Deterministic Policy Gradients (DDPG). We will include implementations of these reinforcement learning models in the 'Getting Started' tutorial provided to competitors. The tutorial will include key insights from solutions from the competitors from the last challenge.

%This competition will fuse biomechanics, computer science, neuroscience, and medical research to explore a grand challenge in human movement, motor control, and prosthetics. The entire competition is built on free and open source components coming from academics. Competitors will be required to tackle major challenges in reinforcement learning: large dimensionality of action space, delayed sensing and actuation, meta-learning, and multi-task learning. Controllers that can synthesize realistic movement will directly help design, prototype and tune prosthetics.

\subsection{Background and scope}\label{ss:scope}

%Technological advancements have greatly increased the potential of devices in improving human movement. These devices span a wide range of designs and tasks, including prosthetics aimed at restoring mobility for impaired individuals, and passive and active devices that are targeted at augmenting able-bodied individuals. Designing these devices and tuning them, however, continue to be difficult tasks that slow down progress in the field. Experiments are time-consuming and costly, and we lack a fundamental understanding of how these devices will interact with humans, changing both their movement patterns and their neural patterns. Furthermore, these devices have varied success among many people that is not well-characterized.

Using biomechanical simulations to analyze experimental data has led to novel insights about human-device interaction. For example, one group used simulations to study a device that decreased the force that the ankle needed to produce during hopping but, paradoxically, did not reduce energy expenditure. Simulations that included a sophisticated model of muscle-tendon dynamics revealed that this paradox occurred because the muscles were at a length that was less efficient for force production \cite{farris2014exo}. Another study used simulations of running to calculate ideal device torques needed to reduce energy expenditure during running\cite{uchida2016device}, and insights gained from that study were used to decrease the metabolic cost in experimental studies \cite{lee2017exosuit}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.72	\linewidth]{img2018/00_intro/prost.png}
\caption{A patient with a prosthetic leg (left); musculoskeletal simulation of a patient with a prosthetic leg as modeled in Stanford's OpenSim software (right).}
\label{fig:running}
\end{figure}

A limitation of the previous studies, however, is that they used the kinematics from the experiments as a constraint. Since assistive devices may greatly change one's kinematics, these analyses cannot predict the neural and kinematic adaptations induced by these devices on the human. Instead, we require a framework that can generate simulations of gait that can adapt realistically to various perturbations. This framework, for instance, would help us understand the complex motor control and adaptations necessary to control both a healthy human and one with a prosthetic.

%Understanding motor control is a grand challenge in biomechanics and neuroscience. One of the greatest hurdles is the complexity of the neuromuscular control system. Muscles are complex actuators whose forces are dependent on their length, velocity, and activation level, and these forces are then transmitted to the bones through a compliant tendon. Coordinating these musculotendon actuators to generate a robust motion is further complicated by delays in the biological system, including sensor delays, control signal delays, and muscle-tendon dynamics. 

Recent advances in reinforcement learning, biomechanics, and neuroscience enable us to build a framework that tackles these limitations. The biomechanics community has developed models and controllers for different movement tasks, two of which are particularly relevant for this challenge. The first study developed a model and controller that could walk, turn, and avoid obstacles \cite{song2015neural}. The second study generated simulated walking patterns at a wide range of target speeds that reproduced many experimental measures, including energy expenditure \cite{ong2017walking}. These controllers, however, are limited to generating walking and running and need domain expertise to design.

Modern reinforcement learning techniques have been used recently to train more general controllers in locomotion. Controllers generated using these techniques have the advantage that, compared to the gait controllers previously described, less user input is needed to hand-tune the controllers, and they are more flexible in their ability to learn additional, novel tasks. For example, reinforcement learning has been used to train controllers for locomotion of complicated humanoid models \cite{lillicrap2015continuous,schulman2015trust}. Although these methods find solutions without domain specific knowledge, the resulting motions are not realistic, possibly because these models do not use biologically accurate actuators.

Through the challenge, we aimed to investigate if deep reinforcement learning methods can yield more realistic results with biologically accurate models of the human musculoskeletal system. We designed the challenge so that it stimulates research at the intersection of reinforcement learning, biomechanics, and neuroscience, encouraging development of methods appropriate for environments characterized by the following: 1) a high-dimensional action space, 2) a complex biological system, including delayed actuation and complex muscle-tendon interactions, 3) a need for a flexible controller for an unseen environment, and 4) an abundance of experimental data that can be leveraged to speed up the training process.

%OpenSim is an open-source software environment which implements computational biomechanical models and allows muscle-driven simulations of these models \cite{delp2007opensim}. It is a flexible platform that can be easily incorporated into an optimization routine using reinforcement learning.

%We additionally are helping advance open source tools for research. Our environment is setup using an open-source physics engine--a potential alternative for commercial closed-source MuJoCo \cite{todorov2012mujoco}, which is widely used in the reinforcement learning research community. Similarly, crowdAI.org\footnote{\url{https://crowdai.org/}}--the platform on which the challenge will be run--is also an open-source alternative to Kaggle\footnote{\url{https://kaggle.com/}}. Thanks to the agile infrastructure of crowdAI.org and components from OpenAI reinforcement learning environments\footnote{\url{https://github.com/kidzik/osim-rl-grader}}, we managed to seamlessly integrate the reinforcement learning setting (which is not available in Kaggle).

%\tblue{This challenge is particularly relevant to the NIPS community as it brings together neuroscience and computer science. We anticipate competitors with expertise in biomechanics, robotics, deep learning, reinforcement learning, and computational neuroscience. Participants in the previous challenge emphasized that it was a great learning experience at the intersection of multiple fields}\footnote{\url{https://medium.com/mlreview/our-nips-2017-learning-to-run-approach-b80a295d3bb5}}, and we have designed this current challenge in a similar manner.

%\tblue{With the great interest from last year, our more extensive channels for promotion, and a compelling, medically focused application, we are anticipating twice as many participants (i.e., around 1000). Several features of the competition will ensure a large audience. First, entries in the competition will produce engaging (and sometimes comical) visuals of a humanoid moving through a complex environment. Second, we will supply participants with an environment that is easy to set-up and get started, without extensive knowledge of biomechanics. Third, we will re-engage the community from the previous challenge}\footnote{\url{https://gitter.im/crowdAI/NIPS-Learning-To-Run-Challenge\#utm_source=notification&utm_medium=email\&utm_campaign=unread-notifications}}.

%The competition was designed for participants to use reinforcement learning methods to create their controllers. However, unlike in pure reinforcement learning tasks, we allowed participants to use publicly available human movement data.

\subsection{Task}\label{ss:task}

Competitors were tasked with building a real-time controller for a simulated agent to walk or run at a requested speed and direction. The task was designed in a typical reinforcement learning setting \cite{Sutton1999} in which an agent (musculoskeletal model) interacts with an environment (physics simulator) by taking actions (muscle excitations) based on observations (a function of the internal state of the model) in order to maximize the reward.

\textbf{Agent and observations.} The simulated agent was a musculoskeletal model of a human with a prosthetic leg. The model of the agent included $19$ muscles to control $14$ degrees-of-freedom (DOF). At every iteration the agent received the current observed state, a vector of consisting of $406$ values: ground reaction forces, muscle activities, muscle fiber lengths, muscle velocities, tendon forces, and positions, velocities, and accelerations of joint angles and body segments.

Compared to the original model from \cite{ong2017walking} we allowed the hip to abduct and adduct, and the pelvis to move freely in space. To control the extra hip degrees of freedom, we added a hip abductor and adductor to each leg, which added 4 muscles total. The prosthesis replaced the right tibia and foot, and we removed the 3 muscles that cross the ankle for that leg. Table \ref{tbl:action} lists all muscles in the model. 

\begin{table}[h!]
\setlength\tabcolsep{0.25cm}
\setlength{\extrarowheight}{.2em}
\centering
\begin{tabular}{r l l l } 
Name & Side	& Description &	Primary function(s)\\
 \hline
abd & both & Hip abductors & Hip abduction (away from body’s vertical midline)\\
add & both & Hip adductors & Hip adduction (toward body’s vertical midline)\\
bifemsh & both & Short head of the biceps femoris &	Knee flexion\\
gastroc & left & Gastrocnemius & Knee flexion and ankle extension (plantarflexion)\\
glut\_max & both &	Gluteus maximus & Hip extension\\
hamstrings & both &	Biarticular hamstrings & Hip extension and knee flexion\\
iliopsoas & both &	Iliopsoas &	Hip flexion\\
rect\_fem &	both & Rectus femoris &	Hip flexion and knee extension\\
soleus & left &	Soleus & Ankle extension (plantarflexion)\\
tib\_ant & left & Tibialis anterior & Ankle flexion (dorsiflexion)\\
vasti & both & Vasti & Knee extension\\
\end{tabular}
\caption{A list of muscles that describe the action space in our physics environment. Note that some muscles are missing in the amputated leg (right).}
\label{tbl:action}
\end{table}

\textbf{Actions and environment dynamics.} Based on the observation vector of internal states, each participant's controller would output a vector of muscle excitations (see Table \ref{tbl:action} for the list of all muscles). The physics simulator, OpenSim, calculated muscle activations from excitations using first-order dynamics equations. Muscle activations generate movement as a function of muscle properties such as strength, and muscle states such as current length, velocity, and moment arm. An overall estimate of muscle effort was calculated using the sum of muscle activations squared, a commonly used metric in biomechanical studies \cite{crowninshield1981, thelen2003cmc}. Participants were evaluated by overall muscle effort and the distance between the requested and observed velocities.

%Feasibility of our problem is assured by the successful run of the previous challenge\footnote{\url{https://www.crowdai.org/challenges/learning-to-run}}. We will make sure that the methods used by top participants in the previous challenge are sufficient as a starting step for the lowest difficulty. In order to tune the difficulty, we will train baseline controllers from the preliminary challenge in the new setup. This will allow us to set the complexity at the right level: stimulating research, yet solvable.

\textbf{Reward function and evaluation.} Submissions were evaluated automatically. In Round 1, participants interacted directly with a remote environment. The overall goal of this round was to generate controls such that the model would move forward at 3 m/s. The total reward was calculated as

$$ \sum_{t=1}^{T} 9 - |v_x(s_t) - 3|^2, $$

where \(s_t\) is the state of the model at time \(t\), \(v_x(s)\) is the horizontal velocity vector of the pelvis in the state \(s\), and \(s_t = M(s_{t-1}, a(s_{t_1}))\), i.e. states follow the simulation given by model \(M\). $T$ is the episode termination time step, which is equal to $1000$ if the model did not fall for the full 10 second duration, or is equal to the first time point when that the pelvis of the model falls below $0.6$ m to penalize falling.

In Round 2, in order to mitigate the risk of overfitting, participants submitted Docker containers so that they could not infer the specifics of the environment by interacting with it. The objective was to move the model according to requested speeds and directions. This objective was measured as a distance between the requested and observed velocity vector.

The requested velocity vector varied during the simulation. We commanded approximately $3$ changes in direction and speed during the simulation. More precisely, let $q_0 = 1.25,r_0 = 1$ and let $N_t$ be a Poisson process with $\lambda = 200$. We define
\[
    q_t = q_{t-1} + \mathbf{1}_{(N_t \neq N_{t-1})} u_{1,t} \text{ and }
    r_t = r_{t-1} + \mathbf{1}_{(N_t \neq N_{t-1})} u_{2,t},
\]
where $\mathbf{1}_{(A)}$ is the indicator function of the event $A$ (here, a jump in the Poisson process). We define $u_{1,t} \sim \mathcal{U}([-0.5,0.5])$ and $u_{2,t} \sim \mathcal{U}([-\pi/8,\pi/8])$, where $\mathcal{U}([a,b])$ denotes a uniform distribution on $[a,b]$ interval.

In order to keep the locomotion as natural as possible, we also added a penalties for overall muscle effort as validated in previous work \cite{crowninshield1981, thelen2003cmc}. The final reward function took form

\[
\sum_{t=1}^{T} \left( 10 - |v_x(s_t) - w_{t,x} |^2 - |v_z(s_t) - w_{t,z} |^2 - 0.001\sum_{i=1}^{d}a_{t,i}^2 \right),
\]
where $w_{t,x}$ and $w_{t,z}$ correspond to $q_t$ and $r_t$ expressed in Cartesian coordinates,  $T$ is termination step of the episode as described previously, $a_{t,i}$ is the activation of muscle $i$ at time $t$, and $d$ is the number of muscles.

%\textbf{Difficulty parametrization.} Environments were parametrized by two parameters: \verb|difficulty| and \verb|seed|. Difficulty corresponds to the number and density of obstacles as well as variability in the requested velocities. The \verb|seed| is a number which uniquely identifies pseudo-random generation of the obstacles positions in the environment and should be leveraged in training to obtain a robust controller. The seed ranges between $0$ and $2^{63} - 1$. Both \verb|seed| and \verb|difficulty| of the final test environment are unknown to participants. Such setup allowed us to give access to infinitely many training environments, as well as to choose the final difficulty reactively, depending on users' performance leading up to the final competition round.

Since the environment is subject to random noise, submissions were tested over ten trials and the final score was the average from these trials.

\subsection{Solutions}\label{ss:solutions}

Our challenge attracted 425 teams who submitted 4,575 solutions. The top 50 teams from Round~1 qualified for Round~2. In Table \ref{tbl:leaderboard} we list the top teams from Round~2. Detailed descriptions from each team are given in the subsequent sections of this article. Teams that achieved 1st through 10th place described their solutions in sections 2 through 11. Two other teams submitted their solutions as well (Sections 12 and 13).

\begin{table}[h!]
\setlength\tabcolsep{0.25cm}
\setlength{\extrarowheight}{.2em}
\centering
\begin{tabular}{r | l l l l l } 
  & Team & Score & \# entries & Base algorithm\\
 \hline
 1 & Firework       & 9981 & 10 & DDPG \\ 
 2 & NNAISENSE      & 9950 & 10 & PPO  \\
 3 & Jolly Roger    & 9947 & 10 & DDPG  \\
 4 & Mattias       & 9939 & 10 & DDPG  \\
 5 & ItsHighNoonBangBangBang         & 9901 & 3  & DDPG  \\
 6 & jbr            & 9865 & 9  & DDPG  \\ 
 7 & Lance          & 9853 & 4  & PPO \\
 8 & AdityaBee      & 9852 & 10 & DDPG  \\
 9 & wangzhengfei   & 9813 & 10 & PPO  \\
 10 & Rukia         & 9809 & 10 & PPO  \\
\end{tabular}
\caption{Final leaderboard (Round 2).}
\label{tbl:leaderboard}
\end{table}

In this section we highlight similarities and differences in the approaches taken by the teams. Of particular note was the amount of compute resources used by the top participants. Among the top ten submissions, the highest amount of resources reported for training the top model was 130,000 CPU-hours, while the most compute-efficient solution leveraged experimental data and imitation learning (Section~\ref{s:lance}) and took only 100 CPU-hours to achieve 7th place in the challenge (CPU-hours were self-reported). Even though usage of experimental data was allowed in this challenge, most participants did not use it and focused only on reinforcement learning with a random starting point. While such methods are robust, they require very large compute resources. 

While most of the teams used variations of well-established algorithms such as DDPG and PPO, each team used a combination of other strategies to improve performance. We identify some of the key strategies used by teams below.\\
\ \newline
\noindent\textbf{Leveraging the model.} Participants used various methods to encourage the model to move in a realistic way based on observing how humans walk. This yielded good results, likely due to the realistic underlying physics and biomechanical models. Specific strategies to leverage the model include the following:
\begin{itemize}
    \item Reward shaping: Participants modified the reward for training in such a way that it still makes the model train faster for the actual initial reward. (see, for example, Sections \ref{sss:reward-jolly}, \ref{sss:reward-mattias}, or \ref{sss:reward-itshigh}).
    \item Feature engineering: Some of the information in the state vector might add little value to the controller, while other information can give a stronger signal if a non-linear mapping based on expert knowledge is applied first (see, for example, Sections \ref{sss:reward-jolly}, \ref{sss:observation-mattias}, or \ref{sss:observation-jbr}). Interestingly, one team achieved a high score without feature engineering (Section \ref{sss:large-space}).
    \item Human-in-the-loop optimization: Some teams first trained a batch of agents, then hand picked a few agents that performed well for further training (Section \ref{sss:human-in-the-loop}).
    \item Imitation learning: One solution used experimental data to quickly find an initial solution and to guide the controller towards typical human movement patterns. This resulted in training that was quicker by a few orders of magnitude (Section \ref{s:lance}).
\end{itemize}
\ \newline
\noindent\textbf{Speeding up exploration.} In the early phase of training, participants reduced the search space or modified the environment to speed up exploration using the following techniques:
\begin{itemize}
    \item Frameskip: Instead of sending signals every $1/100$ of a second (i.e., each frame), participants sent the same control for, for example, 5 frames. Most of the teams used some variation of this technique (see, for example, Section \ref{sss:observation-mattias})
    \item Sample efficient algorithms: all of the top teams used algorithms that are known to be sample-efficient, such as PPO and DDPG. 
    \item Exploration noise: Two main exploration strategies involved adding Gaussian or Ornstein--Uhlenbeck noise to actions (see Section \ref{sss:parameter-jolly}) or parameter noise in the policy (see Section \ref{s:nnaisense} or \ref{sss:parameter-itshigh}).
    \item Binary actions: Some participants only used muscle excitations of exactly 0 or 1 instead of values in the interval $[0,1]$ (``bang-bang'' control) to reduce the search space (Section \ref{sss:large-space}).
    \item Time horizon correction: An abrupt end of the episode due to a time limit can potentially mislead the agent. To correct for this effect, some teams used an estimate of the value behind the horizon from the value function (see Section \ref{sss:time-horizon}).
    \item Concatenating actions: In order to embed history in the observation, some teams concatenated observations before feeding them to the policy (Section \ref{sss:concatenation}).
    \item Curriculum learning: Since learning the entire task from scratch is difficult, it might be advantageous to learn low-level tasks firsts (e.g., bending the knee) and then learn high-level tasks (e.g., coordinating muscles to swing a leg) (Section \ref{ss:methodology})
    \item Transfer learning: One can consider walking at different speeds as different subtasks of the challenge. These subtasks may share control structure, so the model trained for walking at 1.25 m/s may be retrained for walking at 1.5 m/s etc. (Section \ref{ss:methodology})
\end{itemize}
\ \newline
\noindent\textbf{Speeding up simulations.} Physics simulations of muscles and ground reaction forces are computationally intensive. Participants used the following techniques to mitigate this issue: 
\begin{itemize}
    \item Parallelization: Participants ran agents on multiple CPUs. A master node, typically with a GPU, was collecting these experiences and updating weights of policies. This strategy was indispensable for success and it was used by all teams (see, for example, Sections \ref{sss:distributed-jolly}, \ref{sss:distributed-apex}, \ref{sss:distributed-jbr} or  \ref{sss:distributed-shawk})
    \item Reduced accuracy: In OpenSim, the accuracy of the integrator is parameterized and can be manually set before the simulation. In the early stage of training, participants reduced accuracy to speed up simulations to train their models more quickly. Later, they fine-tuned the model by switching the accuracy to the same one used for the competition \cite{kidzinski2018learning}.
\end{itemize}
\ \newline
\noindent\textbf{Fine-tuning.} A common statistical technique for increasing the accuracy of models is to output a weighted sum of multiple predictions. This technique also applies to policies in reinforcement learning, and many teams used some variation of this approach: ensemble of different checkpoints of models (Section \ref{sss:ensemble}), training multiple agents simultaneously (Section \ref{s:mattias}), or training agents with different seeds (Section \ref{s:jbr}).\\
\ \newline
While this list covers many of the commonly used strategies, a more detailed discussion of each team's approach is detailed in the following sections.

%\subsubsection{Differences}

%Time horizon correction (Section \ref{sss:time-horizon}).
%Very light feature engineering --- Large number of features (Section \ref{sss:large-space}).
%Bang-bang control (Section \ref{sss:large-space}).
%Sergey: quantile value distribution, concatenation of states\\
%Lance: Imitation learning
%\textbf{.}



==> sections2018/00_template.tex <==
\section{TEMPLATE: [One sentence title of your solution]}\label{s:template}
\sectionauthor{[names of team members]}

One paragraph summary of your approach including: the key algorithm (PPO, DDPG, etc?), important tricks, results and lessons learned.

\subsection{Methods}

Methods you used
\begin{itemize}
    \item Hyper-parameters
    \item Parallel computing framework
    \item Hardware you used
\end{itemize}

\subsection{Experiments and results}

Technical details and results:
\begin{itemize}
    \item Hyper-parameters
    \item Parallel computing framework
    \item Hardware you used
\end{itemize}
\subsection{Discussion}

\begin{enumerate}
\item What went well?
\item What could you improve?
\end{enumerate}
